A sequential solution to the density classification task using an intermediate alphabet

We present a sequential cellular automaton of radius 2 1 as a solution to the density classification task that makes use of an intermediate alphabet, and converges to a clean fixed point with no remaining auxiliary or intermediate information. We extend this solution to arbitrary finite alphabets and to configurations in higher dimensions.

==> parts/exec2DIEEE.tex <==
\scalebox{0.8}{
\begin{tikzpicture}
  \newcommand{\xgap}{0.9}
  \newcommand{\ygap}{1.4}
  \newcommand{\largexgap}{3.1cm}
  \newcommand{\largeygap}{-4.8cm}

  \begin{scope}[xshift=\largexgap * 0, yshift=\largeygap * 0]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %values
    \foreach \x\y\nodetext
    in {
      0/0/2, 1/0/2, 2/0/0,
      0/1/1, 1/1/2, 2/1/2,
      0/2/0, 1/2/1, 2/2/0
    }
    {
      \draw (\x * \xgap, \y * \ygap) node {\nodetext};
    }
  \end{scope}

  \begin{scope}[xshift=\largexgap * 1, yshift=\largeygap * 0]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %S values
    \draw (0 * \xgap, 2 * \ygap) node {0};

    %Intermediate values
    \foreach \x\y\tapesymbol\memory
    in {
      0/0/2/S, 1/0/2/S, 2/0/0/S,
      1/1/X/S, 2/1/2/S,
      1/2/X/\{1\}
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$\begin{matrix}
          \circ \\
          \tapesymbol \\
          \memory
        \end{matrix}$};
    }

    %Manual values
    \draw (0 * \xgap, 1 * \ygap)
      node {$\begin{matrix}
        \circ \\
        1 \\
        \{0, 1\}
      \end{matrix}$};

    \draw (2 * \xgap, 2 * \ygap)
      node {$\begin{matrix}
        \circ \\
        X \\
        \{0, 1\}
      \end{matrix}$};
  \end{scope}

  \begin{scope}[xshift=\largexgap * 2, yshift=\largeygap * 0]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %Isolated value
    \draw (0 * \xgap, 2 * \ygap)
      node {$\begin{matrix}
        \circ \\
        0 \\
        S
      \end{matrix}$
    };

    %Intermediate values
    \foreach \x\y\tapesymbol\memory
    in {
      2/0/X/S,
      0/1/X/\{1\}, 1/1/X/\{1\},
      1/2/X/\emptyset, 2/2/X/\emptyset
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$\begin{matrix}
          \bullet \\
          \tapesymbol \\
          \memory
        \end{matrix}$};
    }

    %Manual values
    \draw (0 * \xgap, 0 * \ygap)
      node {$\begin{matrix}
        \bullet \\
        2 \\
        \{1, 2\}
      \end{matrix}$};

    \draw (1 * \xgap, 0 * \ygap)
      node {$\begin{matrix}
        \bullet \\
        2 \\
        \{1, 2\}
      \end{matrix}$};

    \draw (2 * \xgap, 1 * \ygap)
      node {$\begin{matrix}
        \bullet \\
        X \\
        \{1, 2\}
      \end{matrix}$};
  \end{scope}

  \begin{scope}[xshift=\largexgap * 0, yshift=\largeygap * 1]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %Isolated value
    \draw (0 * \xgap, 2 * \ygap)
      node {$\begin{matrix}
        \bullet \\
        0 \\
        S
      \end{matrix}$
    };

    %Intermediate values
    \foreach \x\y\tapesymbol\memory
    in {
      0/0/X/\{2\}, 1/0/2/\{2\}, 2/0/X/\{2\},
      0/1/X/\emptyset, 1/1/X/\emptyset, 2/1/X/\emptyset,
      1/2/X/\emptyset, 2/2/X/\emptyset
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$\begin{matrix}
          \circ \\
          \tapesymbol \\
          \memory
        \end{matrix}$};
    }
  \end{scope}

  \begin{scope}[xshift=\largexgap * 1, yshift=\largeygap * 1]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %Isolated value
    \draw (0 * \xgap, 2 * \ygap)
      node {$\begin{matrix}
        \circ \\
        X \\
        \{0, 2\}
      \end{matrix}$
    };

    %Intermediate values
    \foreach \x\y\tapesymbol\memory
    in {
      0/0/X/\emptyset, 1/0/X/\{2\}, 2/0/X/\{2\},
      0/1/X/\emptyset, 1/1/X/\emptyset, 2/1/X/\emptyset,
      1/2/X/\emptyset, 2/2/X/\emptyset
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$\begin{matrix}
          \bullet \\
          \tapesymbol \\
          \memory
        \end{matrix}$};
    }
  \end{scope}

  \begin{scope}[xshift=\largexgap * 2, yshift=\largeygap * 1]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %Isolated value
    \draw (0 * \xgap, 2 * \ygap)
      node {$\begin{matrix}
        \bullet \\
        X \\
        \{2\}
      \end{matrix}$
    };

    %S values
    \foreach \x\y\tapesymbol\memory
    in {
      0/0, 1/0, 2/0,
      0/1, 1/1, 2/1,
      1/2, 2/2
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$2$};
    }
  \end{scope}

  \begin{scope}[xshift=\largexgap * 0, yshift=\largeygap * 2]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %S values
    \foreach \x\y\tapesymbol\memory
    in {
      0/0, 1/0, 2/0,
      0/1, 1/1, 2/1,
      0/2, 1/2, 2/2
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$2$};
    }
  \end{scope}

  \begin{scope}[xshift=\largexgap * 2, yshift=\largeygap * 2]
    %grid
    \draw[gray!50!white] foreach \x in {0, ..., 3} {
      (\x * \xgap - \xgap / 2, - \ygap / 2) -- (\x * \xgap - \xgap / 2, \ygap * 2.5)
    };
    \draw[gray!50!white] foreach \y in {0, ..., 3} {
      (- \xgap / 2, \y * \ygap - \ygap / 2) -- (\xgap * 2.5, \y * \ygap - \ygap / 2)
    };

    %coordinates
    \foreach \x\y\ry
    in {
      0/0/2, 1/0/2, 2/0/2,
      0/1/1, 1/1/1, 2/1/1,
      0/2/0, 1/2/0, 2/2/0
    }
    {
      \draw (\x * \xgap, \y * \ygap)
        node {$(\x, \ry)$};
    }
  \end{scope}

\end{tikzpicture}
}


==> parts/table1IEEE.tex <==
{\tabulinesep=1.2mm
\begin{tabu}{ | c | c | } 
  \hline
  \bf{Case name} & \bf{Pattern} \\
  \hline
  % FIXED POINT
  Fixed point behaviour & $00 \mapsto 0$, $11 \mapsto 1$ \\
  \hline
  % KICKSTART
  Kickstart &
  0 1 $\mapsto \begin{psmallmatrix} \circ \\ X \\ \{1\} \end{psmallmatrix}$,
  1 0 $\mapsto \begin{psmallmatrix} \circ \\ X \\ \{0\} \end{psmallmatrix}$ \\
  \hline
  % #1 PROPAGATION, REMOVING
  \begin{tabular}{@{}c@{}} First propagation phase\\and removing a character\end{tabular} &
  $\begin{smallmatrix}\forall M \subseteq \B,\\b \in \B \setminus M,\\c \in \{\bullet, \circ\},\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ M \end{psmallmatrix}\ b
  \mapsto
  \begin{psmallmatrix} c \\ X \\ M \cup \{b\} \end{psmallmatrix}$
  \\
  \hline
  % #1 PROPAGATION, NOT REMOVING
  \begin{tabular}{@{}c@{}} First propagation phase,\\ without removing\\a character\end{tabular} &
  $\begin{smallmatrix}\forall M \subseteq \B,\\b \in M,\\c \in \{\bullet, \circ\},\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ M \end{psmallmatrix}\ b
  \mapsto
  \begin{psmallmatrix} c \\ b \\ M \end{psmallmatrix}$
  \\
  \hline
  % SWAP, MEMORY RESET
  \begin{tabular}{c} Swap phase and\\ resetting the memory \end{tabular} &
  $\begin{smallmatrix}\forall c, c' \in \{\bullet, \circ\},\\c \neq c',\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ \B \end{psmallmatrix}
  \begin{psmallmatrix} c \\ ? \\ ? \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} c' \\ X \\ \emptyset \end{psmallmatrix}$
  \\
  \hline
  % PROPAGATION, REMOVING
  \begin{tabular}{c} Propagation phase and\\ removing a character\end{tabular} &
  $\begin{smallmatrix}\forall M \subseteq \B,\\b \in \B \setminus M,\\c, c' \in \{\bullet, \circ\},\\c \neq c',\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ M \end{psmallmatrix}
  \begin{psmallmatrix} c' \\ b \\ ? \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} c \\ X \\ M \cup \{b\} \end{psmallmatrix}$
  \\
  \hline
  % PROPAGATION, WITHOUT REMOVING
  \begin{tabular}{@{}c@{}} Propagation phase,\\without removing\\a character\end{tabular} &
  $\begin{smallmatrix}\forall M \subseteq \B,\\b \in \B \setminus M,\\c, c' \in \{\bullet, \circ\},\\c \neq c',\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ M \end{psmallmatrix}
  \begin{psmallmatrix} c' \\ b \\ ? \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} c \\ b \\ M \end{psmallmatrix}$
  \\
  \hline
  % SWAP, CONVERGENCE
  \begin{tabular}{c} Swap phase and\\ starting the convergence\end{tabular} &
  $\begin{smallmatrix}\forall b \in \B,\\c \in \{\bullet, \circ\},\end{smallmatrix}$
  $\begin{psmallmatrix} c \\ ? \\ \{b\} \end{psmallmatrix}
  \begin{psmallmatrix} c \\ ? \\ ? \end{psmallmatrix}
  \mapsto b$
  \\
  \hline
  Convergence phase &
  $\forall b \in \B,$
  $b\ 
  \begin{psmallmatrix} ? \\ ? \\ ? \end{psmallmatrix}
  \mapsto b$
  \\
  \hline
\end{tabu}
}

==> parts/table2IEEE.tex <==
{\tabulinesep=1.2mm
\begin{tabu}{ | c | c | c | } 
  \hline
  \bf{Case name} & \bf{Example} \\
  \hline
  % FIXED POINT
  Fixed point behaviour & $00 \mapsto 0$ \\
  \hline
  % KICKSTART
  Kickstart &
  0 1 $\mapsto \begin{psmallmatrix} \circ \\ X \\ \{1\} \end{psmallmatrix}$ \\
  \hline
  % #1 PROPAGATION, REMOVING
  \begin{tabular}{@{}c@{}} First propagation phase\\and removing a character\end{tabular} &
  $\begin{psmallmatrix} \circ \\ 0 \\ \{0\} \end{psmallmatrix}\ 1
  \mapsto
  \begin{psmallmatrix} \circ \\ X \\ \B \end{psmallmatrix}$
  \\
  \hline
  % #1 PROPAGATION, NOT REMOVING
  \begin{tabular}{@{}c@{}} First propagation phase,\\ without removing\\a character\end{tabular} &
  $\begin{psmallmatrix} \bullet \\ 1 \\ \{1\} \end{psmallmatrix}\ 1
  \mapsto
  \begin{psmallmatrix} \bullet \\ 1 \\ \{1\} \end{psmallmatrix}$
  \\
  \hline
  % SWAP, MEMORY RESET
  \begin{tabular}{c} Swap phase and\\ resetting the memory \end{tabular} &
  $\begin{psmallmatrix} \bullet \\ X \\ \B \end{psmallmatrix}
  \begin{psmallmatrix} \bullet \\ X \\ \{0\} \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} \circ \\ X \\ \emptyset \end{psmallmatrix}$
  \\
  \hline
  % PROPAGATION, REMOVING
  \begin{tabular}{c} Propagation phase and\\ removing a character\end{tabular} &
  $\begin{psmallmatrix} \bullet \\ X \\ \emptyset \end{psmallmatrix}
  \begin{psmallmatrix} \circ \\ 1 \\ \B \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} \bullet \\ X \\ \{1\} \end{psmallmatrix}$
  \\
  \hline
  % PROPAGATION, WITHOUT REMOVING
  \begin{tabular}{@{}c@{}} Propagation phase,\\without removing\\a character\end{tabular} &
  $\begin{psmallmatrix} \circ \\ X \\ \B \end{psmallmatrix}
  \begin{psmallmatrix} \bullet \\ X \\ \{0\} \end{psmallmatrix}
  \mapsto
  \begin{psmallmatrix} \circ \\ X \\ \B \end{psmallmatrix}$
  \\
  \hline
  % SWAP, CONVERGENCE
  \begin{tabular}{c} Swap phase and\\ starting the convergence\end{tabular} &
  $\begin{psmallmatrix} \circ \\ 0 \\ \{0\} \end{psmallmatrix}
  \begin{psmallmatrix} \circ \\ X \\ \emptyset \end{psmallmatrix}
  \mapsto 0$
  \\
  \hline
  Convergence phase &
  $1\ 
  \begin{psmallmatrix} \circ \\ 1 \\ \B \end{psmallmatrix}
  \mapsto 1$
  \\
  \hline
\end{tabu}
}
